Human-instructed Deep Hierarchical Generative Learning for Automated Urban Planning

The essential task of urban planning is to generate the optimal land-use configuration of a target area. However, traditional urban planning is time-consuming and labor-intensive. Deep generative learning gives us hope that we can automate this planning process and come up with the ideal urban plans. While remarkable achievements have been obtained, they have exhibited limitations in lacking awareness of: 1) the hierarchical dependencies between functional zones and spatial grids; 2) the peer dependencies among functional zones; and 3) human regulations to ensure the usability of generated configurations. To address these limitations, we develop a novel human-instructed deep hierarchical generative model. We rethink the urban planning generative task from a unique functionality perspective, where we summarize planning requirements into different functionality projections for better urban plan generation. To this end, we develop a three-stage generation process from a target area to zones to grids. The first stage is to label the grids of a target area with latent functionalities to discover functional zones. The second stage is to perceive the planning requirements to form urban functionality projections. We propose a novel module: functionalizer to project the embedding of human instructions and geospatial contexts to the zone-level plan to obtain such projections. Each projection includes the information of land-use portfolios and the structural dependencies across spatial grids in terms of a specific urban function. The third stage is to leverage multi-attentions to model the zone-zone peer dependencies of the functionality projections to generate grid-level land-use configurations. Finally, we present extensive experiments to demonstrate the effectiveness of our framework.

==> introduction1.tex <==
%urban planning is important ---> bad urban plan will cause expensive cost ---> objective and unbiased perspective leads to benefits.
\vspace{-0.25cm}
\section{Introduction}
% \noindent\textbf{Background and Application Contexts.} 
Urban planning studies urban resources (\textit{e.g.} park, school) allocation, which impacts the design and future development of an area.
Conceptually, urban experts plan a multi-year project to renovate a target area in order to develop a promising community, which includes exploration, feasibility studies, master planning, zone planning, land use planning, and implementation. 
If the created urban plan is inadequate, not only these years but also billions of dollars will be wasted according to the study  ~\cite{litman2015analysis}. 
Thus, how to employ cutting-edge Artificial Intelligence (AI) technologies to alleviate the arduous workloads of urban experts and assist them in generating unbiased and inspiring urban designs has garnered considerable interest.

\begin{figure}[!t]
    % \vspace{-0.15cm}
    \centering
    \includegraphics[width=0.9\linewidth]{img/framework_motivation.pdf}
    % \vspace{-0.5cm}
    \captionsetup{justification=centering}
    \vspace{-0.1cm}
    \caption{An urban planner typically first generates a rough sketch of urban planning and then refines it to the detailed urban planning solution. 
    We aim to design an automated urban planner via mimicking such workflow.
    }
    \vspace{-0.7cm}
    \label{fig:framework_motivation}
\end{figure}


% AI for urban planning is a potential way. ---> The merits of AI planner ---> some examples, sidewalks, baidu for xiongan ---> the study problem of our paper.

Various AI technologies have exhibited the  exciting potential to unlock the possibilities of smart urban planning to optimize urban infrastructures and look into the cities of the future worldwide.
For instance, in USA, Sidewalks, a subsidiary of Google, tried to improve the sustainability, economic opportunity, and new mobility of Toronto by AI~\cite{sidewalk}.
Similarly, in China, Baidu signed a strategic collaboration agreement with Hebei province to develop Xiongan New Area into a smart city via AI techniques ~\cite{baidu}.
These suggest that developing AI-assisted generative urban design has become a hot direction for revolutionizing traditional urban planning. 



%The limitations of existing works.
% \noindent\textbf{Application Challenges.} 
Although much efforts have been devoted to AI for automated urban planning ~\cite{ye2021masterplangan,wang2020reimagining},
these AI-based planning are limited in addressing the following issues. 
\textbf{Issue 1: zone-grid planning dependencies.}
For instance, the study in~\cite{wang2020reimagining}  proposed a GAN-based framework to generate urban plan based on geospatial contexts.
However, this method ignores  the hierarchical dependency between zone-level planning (\textit{i.e.}  functional zone segmentation) and grid-level planning (\textit{i.e.} land-use configuration).
Mixed functional zoning always regulates grid-level built environments to ensure the complementarity and sustainability of the grid-level planning. 
\textbf{Issue 2: peer dependencies between functional zones.}
The mutual dependencies of geosocial aspects between functional zones play an inevitable role in complementary and sustainable planning. 
The study in~\cite{shen2020machine} utilized a deep convolutional GAN to fill the urban elements into a well-designed urban sketch to obtain the final planning.
This method supports zone-grid hierarchical generation, yet lacks the modeling structure of peer dependencies among  zones.
\textbf{Issue 3: human instructions.}
Without regulations, deep generative modeling could generate non-usable land-use configurations that lacks a precise planning objective. 
The most reliable regulations  are human instructions, which are in a textual form of  empirical knowledge of domain experts to represent natural intelligence~\cite{dong2018musegan}. 
It is a well-known challenge to develop a human-machine interface so machines can digest and convert human instructions into knowledge to regularize model structures. 

% Our Contributions.



In order to address the aforementioned limitations, we propose a novel Human-\textbf{I}nstructed Deep \textbf{H}ierarchical Generative Framework (\textbf{IHPlanner}). 
This is a cutting-edge practical tool for urban planning, resulting from two reasons: i) Ubiquitous spatiotemporal mobile data (e.g. point-of-interest, social network data) provides sufficient data for IHPlanner training.
ii) Comprehending human instructions and capturing hierarchical dependencies in planning lead IHPlanner to produce practical urban plans.
Compared with prior works, our main contributions are as follows:
\begin{itemize}
    \item \textbf{Casting the automated urban planning as a deep hierarchical generative modeling task}.
Figure \ref{fig:framework_motivation} shows an urban planner firstly complete functional zoning design, then land uses design.
To mimic such human intelligence, our approach firstly generates functional zone design, then generates grid-level land-use configurations.
We found that the hierarchical generation effectively  models the zone-grid planning dependency.
    \item \textbf{Integrating human instructions from planning experts via conditional embedding}. 
We uncover that human instructions from urban planners can be formulated as the generated conditions.
Our strategy to integrate these conditions is to map human instructions and geospatial contexts into two embedding vectors, and concatenate them as the inputs of the planning generation.
The concatenated embedding not only participates in the generation of the zone-level planning but also determines the learning process of functionality projections.
% In this way, human instructions are used to guide the planning process.
    \item \textbf{Functionalizer makes possible the awareness of the peer dependencies between zones}.
We highlight that a land-use configuration can be interpreted as the summary of a set of semantically-rich urban functionality projections. 
We propose a new module, functionalizer, to obtain functionality projections by projecting the embedding of human instructions and geospatial contexts to different functional zones.
Each projection contains the information of land-use portfolios and how land-uses are geographically structured across spatial grids in terms of a specific functionality.
We demonstrate that the peer planning dependencies among zones are converted into the semantic correlations among these projections.
We model the zone-zone peer dependencies by developing multi-attentions over these projections to generate the grid-level planning. 
    \item \textbf{Extensive experiments and case studies to validate the effectiveness of our framework}.
We conduct experiments and case studies based on the geographical data, traffic flow, road map, POIs, and check-in records in real world.
We compare our proposed framework with six advanced deep generative models, and provide visualizations to show the superiority of our framework.
\end{itemize}
 



















